Multimodal Embodied Agents: A Unified Capability-centric Perspective from Computer-Use to Robot-Use

Multimodal agents (MMAs) sustain interaction through reasoning, memory, tools, and feedback, most visibly as computer-use agents, while robotic systems (RSs) couple sensing and actuation under physical dynamics. We define multimodal embodied agents (MMEAs) as goal-directed systems that couple multimodal task reasoning with physical action and revise decisions from the resulting feedback. This raises a central question: what changes when a multimodal agent moves from computer-use to robot-use? We introduce PAPAV, a unified capability-centric framework of five recurring functions: Perceive the current state, Anticipate action effects, Plan a feasible course, Act through an interface or body, and Verify the outcome. Defined by function rather than architecture, these capabilities let PAPAV identify what all three share and then compare MMEAs with MMAs and with RSs. Five physical constraints, from partial observability to unverifiable outcomes, leave fewer choices fixed in advance and less room to reverse errors. Across 64 benchmarks, explicit evaluation centers on Act; only 5 assess Anticipate and 3 assess Verify, leaving both largely hidden behind task success. These constraints also frame the open challenges we identify. PAPAV therefore provides a common basis for designing reliable physical agents and measuring progress across all five capabilities rather than task success alone.

==> sections/1-introduction/evo_tree/clickable_tree.tex <==
% Clickable tree over a PDF background

\RequirePackage{graphicx}
\RequirePackage{overpic}
\RequirePackage{xcolor}
\RequirePackage{hyperref}

% Support classic BibTeX/natbib and biblatex. Input this file after loading
% the bibliography package in the main document.
\makeatletter
\@ifundefined{AtEveryBibitem}{%
  \newcommand{\TreeBibLink}[2]{\hyperlink{cite.#1}{#2}}%
}{%
  \AtEveryBibitem{\hypertarget{treebib:\thefield{entrykey}}{}}%
  \newcommand{\TreeBibLink}[2]{\hyperlink{treebib:#1}{#2}}%
}
\makeatother

\providecommand{\TreeImageFile}{tree.pdf}
\providecommand{\TreeFigureWidth}{\linewidth}
\providecommand{\TreeFigureCaption}{Evolution of multimodal embodied agents.}
\providecommand{\TreeFigureLabel}{fig:clickable-agent-tree}

% Change to \TreeLinksDebugtrue to display link rectangles in red.
\newif\ifTreeLinksDebug
\TreeLinksDebugfalse

% Arguments: BibTeX key, x, y, width, height in overpic units.
\newcommand{\TreePaperLink}[5]{%
  \put(#2,#3){%
    \TreeBibLink{#1}{%
      \ifTreeLinksDebug
        \color{red!55}\framebox(#4,#5){}%
      \else
        \makebox(#4,#5)[lb]{\phantom{X}}%
      \fi
    }%
  }%
}

\newcommand{\ClickableTreeGraphic}{%
  \begingroup
  \hypersetup{hidelinks}%
  \nocite{%
  mclean2026meta,%
  nasiriany2026robocasa365,%
  yang2026robolab,%
  zhang2026assistance,%
  activevla2026,%
  zhao2026dream,%
  tan2025roboos,%
  jiang2026robowm,%
  tacforesight2026,%
  huang2026vla,%
  xvla2026,%
  avavla2025,%
  checkvla2026,%
  zhou2025libero,%
  jiang2025behavior,%
  roboarena2025,%
  robochallenge2025,%
  mu2025robotwin,%
  chen2025robotwin,%
  jangir2025robotarena,%
  hu2024video,%
  robodreamer2024,%
  octo2024,%
  wang2024hpt,%
  black2024pi0,%
  khazatsky2024droid,%
  liu2024okrobot,%
  khanna2024goat,%
  sayplan2023,%
  zhao2023act,%
  pmlr-v205-wu23c,%
  brohan2023rt1,%
  brohan2023rt2,%
  chi2023diffusionpolicy,%
  hughes2022hydra,%
  campos2021orb,%
  shridhar2020alfred,%
  james2020rlbench,%
  rosinol2020kimera,%
  garrett2020pddlstream,%
  zhu2020robosuite,%
  kahn2018composable,%
  anderson2018vision,%
  finn2017deep,%
  mahler2017dexnet,%
  wla2026,%
  worldvlaloop2026,%
  adaptaffordance2026,%
  lu2026bench,%
  hong2026esi,%
  mimir2026,%
  guo2026planar,%
  fu2026cap,%
  rbvla2026,%
  reflectiveplanning2025,%
  han2026robocerebra,%
  unifiedfailure2025,%
  codeasmonitor2024,%
  yang2025embodiedbench,%
  fastinslow2025,%
  gemini2025robotics,%
  evolvevla2025,%
  vlac2025,%
  chen2025emos,%
  interactgen2025,%
  chang2025partnr,%
  aha2024,%
  yang2024safetychip,%
  mandi2024roco,%
  rekep2024,%
  exploreconfident2024,%
  guo2024doremi,%
  du2023successdetectors,%
  huang2023voxposer,%
  driess2023palm,%
  singh2023progprompt,%
  liu2023reflect,%
  liang2023code,%
  song2023llm,%
  ahn2022can,%
  huang2022inner,%
  padmakumar2022teach,%
  chen2025code2video,%
  zheng2026code2world,%
  yuan2026osworld2,%
  cao2026mobiledreamer,%
  tao2026mmsearch,%
  li2026omnigaia,%
  guo2026agent,%
  fu2026video,%
  su2026agentvista,%
  ouyang2026gameworld,%
  luo2026gamecraft,%
  lu2026webgen,%
  li2026worldmodelbench,%
  shou2025showui,%
  agashe2025agents,%
  wu2025osatlas,%
  qin2025ui,%
  mozannar2025magenticui,%
  rawles2025androidworld,%
  yue2025mmmu,%
  tian2025mmina,%
  zheng2025agentstudio,%
  xu2025crab,%
  mayer2025ivispar,%
  nvidia2025pbench,%
  he2024webvoyager,%
  koh2024visualwebarena,%
  xie2024osworld,%
  cheng2024seeclick,%
  liu2024llava,%
  hong2024cogagent,%
  shen2023hugginggpt,%
  hu2023avis,%
  yang2023mm,%
  xu2026roboagent,%
  showuipi2026%
}
  \begin{overpic}[width=\TreeFigureWidth,percent]{\TreeImageFile}
    \TreePaperLink{mclean2026meta}{11.529016}{48.982727}{8.237987}{1.447891}% ID 1 Meta-World+
    \TreePaperLink{nasiriany2026robocasa365}{21.639268}{48.957770}{9.261501}{1.447882}% ID 2 RoboCasa365
    \TreePaperLink{yang2026robolab}{5.363016}{47.235278}{6.690238}{1.447891}% ID 3 RoboLab
    \TreePaperLink{zhang2026assistance}{12.577483}{47.185360}{7.189517}{1.472855}% ID 4 NIABench
    \TreePaperLink{activevla2026}{21.676728}{47.197831}{7.164553}{1.472855}% ID 5 ActiveVLA
    \TreePaperLink{zhao2026dream}{5.662579}{45.363004}{7.189508}{1.472855}% ID 6 Dream.exe
    \TreePaperLink{tan2025roboos}{13.189096}{45.300599}{6.565425}{1.447891}% ID 7 RoboOS
    \TreePaperLink{jiang2026robowm}{21.639268}{45.313092}{9.261501}{1.472846}% ID 8 RoboWM-Bench
    \TreePaperLink{tacforesight2026}{10.505514}{43.515712}{9.261491}{1.447881}% ID 9 TacForeSight
    \TreePaperLink{huang2026vla}{21.664233}{43.615566}{9.261501}{1.472855}% ID 10 VLA-REPLICA
    \TreePaperLink{xvla2026}{6.061992}{41.768262}{6.190977}{1.447882}% ID 11 X-VLA
    \TreePaperLink{avavla2025}{12.527563}{41.768263}{7.214473}{1.472846}% ID 12 AVA-VLA
    \TreePaperLink{checkvla2026}{21.639268}{41.843139}{8.237987}{1.447891}% ID 13 CheckVLA
    \TreePaperLink{zhou2025libero}{10.480549}{39.796146}{9.261491}{1.447881}% ID 14 LIBERO-PRO
    \TreePaperLink{jiang2025behavior}{21.689199}{39.821091}{9.835655}{1.447891}% ID 15 BEHAVIOR Suite
    \TreePaperLink{roboarena2025}{11.504050}{37.923870}{8.237987}{1.472846}% ID 16 RoboArena
    \TreePaperLink{robochallenge2025}{21.689199}{37.923869}{9.286456}{1.447882}% ID 17 RoboChallenge
    \TreePaperLink{mu2025robotwin}{12.502609}{36.051593}{7.214473}{1.472846}% ID 18 RoboTwin
    \TreePaperLink{chen2025robotwin}{21.689199}{35.976707}{8.762221}{1.472846}% ID 19 RoboTwin 2.0
    \TreePaperLink{jangir2025robotarena}{11.354277}{34.079476}{8.237987}{1.472846}% ID 20 RobotArena∞
    \TreePaperLink{hu2024video}{21.739130}{34.179317}{10.235077}{1.447891}% ID 21 Video Pred. Policy
    \TreePaperLink{robodreamer2024}{11.042225}{30.497189}{8.637408}{1.447891}% ID 22 RoboDreamer
    \TreePaperLink{octo2024}{21.676728}{30.472230}{5.142498}{1.472850}% ID 23 Octo
    \TreePaperLink{wang2024hpt}{27.206156}{30.484717}{5.142498}{1.472846}% ID 24 HPT
    \TreePaperLink{black2024pi0}{9.294780}{28.674844}{4.019136}{1.447891}% ID 25 π0
    \TreePaperLink{khazatsky2024droid}{14.187643}{28.674856}{5.541920}{1.472855}% ID 26 DROID
    \TreePaperLink{liu2024okrobot}{21.639268}{28.637405}{7.214482}{1.472846}% ID 27 OK-Robot
    \TreePaperLink{khanna2024goat}{11.603913}{26.740164}{8.063245}{1.447891}% ID 28 GOAT-Bench
    \TreePaperLink{sayplan2023}{8.658211}{24.693160}{6.041190}{1.422927}% ID 29 SayPlan
    \TreePaperLink{zhao2023act}{15.186178}{24.680667}{4.468486}{1.447891}% ID 30 ACT
    \TreePaperLink{pmlr-v205-wu23c}{21.626796}{24.680679}{9.261491}{1.472846}% ID 31 DayDreamer
    \TreePaperLink{brohan2023rt1}{9.020181}{22.858340}{5.142498}{1.472850}% ID 32 RT-1
    \TreePaperLink{brohan2023rt2}{14.686911}{22.833368}{5.042650}{1.447891}% ID 33 RT-2
    \TreePaperLink{chi2023diffusionpolicy}{21.589348}{22.795931}{8.936964}{1.447891}% ID 34 Diffusion Policy
    \TreePaperLink{hughes2022hydra}{14.799245}{20.649053}{4.942792}{1.472846}% ID 35 Hydra
    \TreePaperLink{campos2021orb}{12.053249}{18.552110}{7.688787}{1.472855}% ID 36 ORB-SLAM3
    \TreePaperLink{shridhar2020alfred}{6.261698}{16.455177}{6.790105}{1.472855}% ID 37 ALFRED
    \TreePaperLink{james2020rlbench}{13.600995}{16.405245}{6.166003}{1.472855}% ID 38 RLBench
    \TreePaperLink{rosinol2020kimera}{21.589348}{16.455177}{6.190968}{1.472855}% ID 39 Kimera
    \TreePaperLink{garrett2020pddlstream}{11.429169}{14.557944}{8.337835}{1.447891}% ID 40 PDDLStream
    \TreePaperLink{zhu2020robosuite}{21.589348}{14.607862}{6.665273}{1.447882}% ID 41 robosuite
    \TreePaperLink{kahn2018composable}{6.785932}{10.364055}{13.006037}{1.472855}% ID 42 Composable Predictors
    \TreePaperLink{anderson2018vision}{21.589348}{10.314124}{7.214473}{1.472855}% ID 43 R2R/VLN
    \TreePaperLink{finn2017deep}{7.285213}{8.217185}{12.606615}{1.472855}% ID 44 Deep Visual Foresight
    \TreePaperLink{mahler2017dexnet}{21.589348}{8.341998}{8.237987}{1.447891}% ID 45 Dex-Net 2.0
    \TreePaperLink{wla2026}{49.972952}{46.086962}{10.609534}{1.472855}% ID 46 World-Lang-Action
    \TreePaperLink{worldvlaloop2026}{37.815675}{47.959227}{9.960477}{1.472855}% ID 47 World-VLA-Loop
    \TreePaperLink{adaptaffordance2026}{34.595378}{46.161845}{6.091119}{1.472846}% ID 48 ADAPT
    \TreePaperLink{lu2026bench}{41.235698}{46.161845}{6.540460}{1.472846}% ID 49 IS-Bench
    \TreePaperLink{hong2026esi}{49.997918}{42.517165}{7.214482}{1.422927}% ID 50 ESI-Bench
    \TreePaperLink{mimir2026}{34.982311}{44.302063}{5.142507}{1.447891}% ID 51 Mimir
    \TreePaperLink{guo2026planar}{40.525300}{45.161241}{6.623600}{1.139714}% ID 52 PlanAR
    \TreePaperLink{fu2026cap}{34.595378}{42.492202}{5.242356}{1.472855}% ID 53 CaP-X
    \TreePaperLink{rbvla2026}{49.972952}{44.339502}{9.361349}{1.472855}% ID 54 Rec. Belief VLA
    \TreePaperLink{reflectiveplanning2025}{38.826705}{40.083209}{9.211572}{1.472855}% ID 55 Reflective Plan.
    \TreePaperLink{han2026robocerebra}{50.122746}{40.145622}{8.337835}{1.447891}% ID 56 RoboCerebra
    \TreePaperLink{unifiedfailure2025}{38.202620}{34.191800}{9.561055}{1.447891}% ID 57 Failure Handling
    \TreePaperLink{codeasmonitor2024}{38.327437}{38.136045}{9.586020}{1.447891}% ID 58 Code-as-Monitor
    \TreePaperLink{yang2025embodiedbench}{50.072815}{38.073647}{9.610984}{1.323069}% ID 59 EmbodiedBench
    \TreePaperLink{fastinslow2025}{60.183066}{37.998745}{7.938423}{1.447891}% ID 60 Fast-in-Slow
    \TreePaperLink{gemini2025robotics}{38.115252}{36.101515}{9.785735}{1.472855}% ID 61 Gemini Robotics
    \TreePaperLink{evolvevla2025}{49.972952}{36.051593}{9.261491}{1.472846}% ID 62 EVOLVE-VLA
    \TreePaperLink{vlac2025}{59.671316}{36.014152}{5.142507}{1.472850}% ID 63 VLAC
    \TreePaperLink{chen2025emos}{49.972952}{34.179317}{5.392142}{1.447891}% ID 64 EMOS
    \TreePaperLink{interactgen2025}{55.876842}{34.091950}{7.738716}{1.472855}% ID 65 InteractGen
    \TreePaperLink{chang2025partnr}{58.997300}{40.257965}{6.365719}{1.447882}% ID 66 PARTNR
    \TreePaperLink{aha2024}{35.893478}{30.409822}{4.393593}{1.472855}% ID 67 AHA
    \TreePaperLink{yang2024safetychip}{40.649062}{30.497190}{7.264401}{1.472855}% ID 68 Safety Chip
    \TreePaperLink{mandi2024roco}{50.035355}{30.297476}{5.017685}{1.472855}% ID 69 RoCo
    \TreePaperLink{rekep2024}{55.876842}{30.297482}{5.142498}{1.472850}% ID 70 ReKep
    \TreePaperLink{exploreconfident2024}{35.593924}{28.587484}{12.332015}{1.447882}% ID 71 Explore until Confident
    \TreePaperLink{guo2024doremi}{49.997918}{28.462659}{6.016226}{1.472855}% ID 72 DoReMi
    \TreePaperLink{du2023successdetectors}{36.530069}{24.680669}{11.682959}{1.472855}% ID 73 VLM Success Detect.
    \TreePaperLink{huang2023voxposer}{49.985446}{24.605781}{7.214473}{1.472846}% ID 74 VoxPoser
    \TreePaperLink{driess2023palm}{57.873936}{24.605781}{6.190968}{1.472846}% ID 75 PaLM-E
    \TreePaperLink{singh2023progprompt}{32.336178}{22.658630}{8.237987}{1.472846}% ID 76 ProgPrompt
    \TreePaperLink{liu2023reflect}{40.848764}{22.658630}{7.214482}{1.472846}% ID 77 REFLECT
    \TreePaperLink{liang2023code}{50.035355}{22.608689}{9.910548}{1.472855}% ID 78 Code as Policies
    \TreePaperLink{song2023llm}{33.284783}{20.661538}{8.113173}{1.472855}% ID 79 LLM-Planner
    \TreePaperLink{ahn2022can}{41.734966}{20.649039}{6.166012}{1.472860}% ID 80 SayCan
    \TreePaperLink{huang2022inner}{50.060332}{20.736433}{10.010406}{1.472846}% ID 81 Inner Monologue
    \TreePaperLink{padmakumar2022teach}{60.719783}{20.786351}{6.166003}{1.447882}% ID 82 TEACh
    \TreePaperLink{chen2025code2video}{70.917414}{49.332223}{7.863529}{1.447891}% ID 83 Code2Video
    \TreePaperLink{zheng2026code2world}{80.927815}{49.332223}{9.286465}{1.447891}% ID 84 Code2World
    \TreePaperLink{yuan2026osworld2}{90.738513}{49.332223}{8.237987}{1.447891}% ID 85 OSWorld2.0
    \TreePaperLink{cao2026mobiledreamer}{68.558352}{47.447473}{10.309961}{1.447882}% ID 86 MobileDreamer
    \TreePaperLink{tao2026mmsearch}{80.902849}{47.410028}{10.309961}{1.472855}% ID 87 MMSearch-Plus
    \TreePaperLink{li2026omnigaia}{91.637197}{47.385062}{6.939882}{1.472855}% ID 88 OmniGAIA
    \TreePaperLink{guo2026agent}{70.592883}{45.412934}{8.262951}{1.472855}% ID 89 Agent-SAMA
    \TreePaperLink{fu2026video}{80.877895}{45.537761}{9.461198}{1.447891}% ID 90 Video-MME-v2
    \TreePaperLink{su2026agentvista}{90.913249}{45.537761}{8.237987}{1.447891}% ID 91 AgentVista
    \TreePaperLink{ouyang2026gameworld}{70.567918}{43.615575}{8.237987}{1.472846}% ID 92 GameWorld
    \TreePaperLink{luo2026gamecraft}{80.927815}{43.615566}{10.759311}{1.472855}% ID 93 GameCraft-Bench
    \TreePaperLink{lu2026webgen}{69.544416}{40.320380}{9.286456}{1.447881}% ID 94 WebGen-Bench
    \TreePaperLink{li2026worldmodelbench}{80.877895}{40.320370}{11.333466}{1.447891}% ID 95 WorldModelBench
    \TreePaperLink{shou2025showui}{92.835446}{40.370293}{6.190977}{1.472854}% ID 96 ShowUI
    \TreePaperLink{agashe2025agents}{72.065744}{38.348243}{6.765131}{1.472855}% ID 97 Agent S2
    \TreePaperLink{wu2025osatlas}{80.852929}{38.348252}{8.237987}{1.472846}% ID 98 OS-ATLAS
    \TreePaperLink{qin2025ui}{89.615149}{38.348243}{7.214482}{1.472855}% ID 99 UI-TARS
    \TreePaperLink{mozannar2025magenticui}{71.092151}{36.176412}{7.763681}{1.472855}% ID 100 Magentic-UI
    \TreePaperLink{rawles2025androidworld}{80.778032}{36.176422}{8.762221}{1.472846}% ID 101 AndroidWorld
    \TreePaperLink{yue2025mmmu}{90.289165}{36.176421}{8.237987}{1.472846}% ID 102 MMMU-Pro
    \TreePaperLink{tian2025mmina}{72.764714}{34.179315}{6.066155}{1.672562}% ID 103 MMInA
    \TreePaperLink{zheng2025agentstudio}{80.877895}{34.179324}{8.013307}{1.622633}% ID 104 AgentStudio
    \TreePaperLink{xu2025crab}{89.889748}{34.179315}{6.166003}{1.672562}% ID 105 CRAB
    \TreePaperLink{mayer2025ivispar}{71.791144}{32.207198}{6.914918}{1.447882}% ID 106 iVISPAR
    \TreePaperLink{nvidia2025pbench}{80.827963}{32.207198}{6.490532}{1.447882}% ID 107 PBench
    \TreePaperLink{he2024webvoyager}{70.143547}{30.260037}{8.512586}{1.472846}% ID 108 WebVoyager
    \TreePaperLink{koh2024visualwebarena}{80.877895}{30.260037}{10.309961}{1.472846}% ID 109 VisualWebArena
    \TreePaperLink{xie2024osworld}{91.861876}{30.260037}{7.214473}{1.472846}% ID 110 OSWorld
    \TreePaperLink{cheng2024seeclick}{72.190549}{28.462659}{6.490541}{1.472855}% ID 111 SeeClick
    \TreePaperLink{liu2024llava}{80.877895}{28.462668}{8.237987}{1.472846}% ID 112 LLaVA-Plus
    \TreePaperLink{hong2024cogagent}{89.814851}{28.462659}{7.189517}{1.472855}% ID 113 CogAgent
    \TreePaperLink{shen2023hugginggpt}{70.692746}{24.693163}{8.088200}{1.472855}% ID 114 HuggingGPT
    \TreePaperLink{hu2023avis}{81.027666}{24.718118}{5.167463}{1.547740}% ID 115 AVIS
    \TreePaperLink{yang2023mm}{86.869153}{24.718118}{8.237987}{1.547740}% ID 116 MM-REACT
    \TreePaperLink{xu2026roboagent}{40.187231}{42.492202}{7.588930}{1.472855}% ID 117 RoboAgent
    \TreePaperLink{showuipi2026}{92.111510}{43.615566}{6.914918}{1.472855}% ID 118 ShowUI-π
    % TODO: Show-Harness is not yet present in refs.bib. Add its key to the
    % nocite list above, then uncomment the calibrated link below.
    \TreePaperLink{chen2026showharness}{49.972952}{47.934261}{8.837114}{1.472855}% ID 119 Show-Harness
  \end{overpic}%
  \endgroup
}

\newcommand{\ClickableTreeFigure}{%
  \begin{figure}[!htbp]
    \centering
    \ClickableTreeGraphic
    \caption{\TreeFigureCaption}
    \label{\TreeFigureLabel}
  \end{figure}%
}

